A Survey on Remote Sensing Foundation Models: From Vision to Multimodality

The rapid advancement of remote sensing foundation models, particularly vision and multimodal models, has significantly enhanced the capabilities of intelligent geospatial data interpretation. These models combine various data modalities, such as optical, radar, and LiDAR imagery, with textual and geographic information, enabling more comprehensive analysis and understanding of remote sensing data. The integration of multiple modalities allows for improved performance in tasks like object detection, land cover classification, and change detection, which are often challenged by the complex and heterogeneous nature of remote sensing data. However, despite these advancements, several challenges remain. The diversity in data types, the need for large-scale annotated datasets, and the complexity of multimodal fusion techniques pose significant obstacles to the effective deployment of these models. Moreover, the computational demands of training and fine-tuning multimodal models require significant resources, further complicating their practical application in remote sensing image interpretation tasks. This paper provides a comprehensive review of the state-of-the-art in vision and multimodal foundation models for remote sensing, focusing on their architecture, training methods, datasets and application scenarios. We discuss the key challenges these models face, such as data alignment, cross-modal transfer learning, and scalability, while also identifying emerging research directions aimed at overcoming these limitations. Our goal is to provide a clear understanding of the current landscape of remote sensing foundation models and inspire future research that can push the boundaries of what these models can achieve in real-world applications. The list of resources collected by the paper can be found in the https://github.com/IRIP-BUAA/A-Review-for-remote-sensing-vision-language-models.

==> tables/vision_language_datasets.tex <==
\begin{table}[!t]
\caption{Comparison with existing remote sensing instruction tuning datasets.}
\label{tab:sample_compare}
\small
\centering
\begin{tabularx}{\textwidth}{lc m{0.4\textwidth} m{0.32\textwidth}}
\toprule
\textbf{Model} & \textbf{\thead{Total \\Sample}} & \textbf{Tasks} & \textbf{Based Datasets}   \\ \hline
RemoteCLIP~\cite{remoteclip} & 166k & Image Caption & RSICD, RSITMD, UCMerced, AUAIR, CARPK, DIOR, DOTA, HRRSD, HRSC, LEVIR, RSOD, Stanford, Visdrone, iSAID, loveDA, Potsdam, Vaihingen \\
SkyCLIP~\cite{skyscript} & 2600k &  & Obtained from Google Earth Engine (GEE) \\
GeoRSCLIP~\cite{georsclip} & 500k & Image Caption & LAION2B-en, LAION400M, LAIONCOCO, COYO700M, CC3M, CC12M, YFCC15M, WIT, Redcaps, SBU, Visual Genome, BigEarthNet, FMoW, MillionAID \\ 
RSGPT~\cite{rsgpt} & 2.6k  & Image Caption & DOTA-v1.5    \\
H$^2$RSVLM~\cite{h2rsvlm}  & 180k & Image Caption, VQA, Multi-Label Scene Classification, Visual Grounding, other basic tasks & DOTA-v2, Fair1M, BANDON, MtS-WH, MSAR, fMoW, CrowdAI, GID, FBP, DeepGlobe, RSVQA, METER-ML, NWPU, RSITMD, UCM, DIOR-RSVG \\
GeoChat~\cite{geochat}  & 318k & Image Caption, Region Caption, VQA, Scene Classification, Visual Grounding, Object Detection, Grounding Description, Multi-Task Conversation & DOTA, DIOR, Fair1M, LRBEN, FloodNet, NWPU-RESISC45   \\
EarthGPT~\cite{earthgpt} & 1005k & Image Caption, Region Caption, VQA, Scene Classification, Visual Grounding, Object Detection, Multi-Task Conversation & RSICD, UCM-Captions, RSITMD, Sydney-Captions, NWPU-Captions, FloodNet, RSVQA-LR, RSIVQA, CRSVQA, NWPU-RESISC45, EuroSAT, UCMerced-Landuse, WHU-RS19, RSSCN7, DSCR, FGSCR-42, DOTA, DIOR, FAR1M, NWPUVHR10, HRRSD, RSOD, UCAS-AOD, VisDrone, AIR-SARShip-2.0, SSDD, HRISD, HIT-UAV, Sea-shipping, Infrared-security, Aerial-mancar, Double-light-vehicle, Oceanic ship, DIOR-RSVG  \\
SkyEyeGPT~\cite{skyeyegpt} & 968k & Image Caption, VQA, Scene Classification, Visual Grounding, UAV Video Caption, Phrase Grounding, Multi-Task Conversation & RSICD, RSITMD, UCM-Captions, Sydney-Captions, NWPU-Captions, CapERA, RSIVQA, RSVQA-LR, RSVQA-HR, RSVG, DIOR-RSVG    \\
LHRS-Bot~\cite{lhrs-bot} & 81.8k & Image Caption, VQA, Scene Classification, Visual Grounding, Multi-Task Conversation & RSITMD, NWPU-Captions, LHRS-Align  \\ 
SkySenseGPT~\cite{skysensegpt} & 1800.8k & Image Caption, Region Caption, VQA, Multi-Label Scene Classification, Object Detection, Multi-Task Conversation, Relation Detection, Relation Reasoning, Object Reasoning, Region-Level SGG, Image-Level SGG & NWPU-RESISC-45, UCM-Landuse, RSITMD, EarthVQA, RSVQA-LR, FloodNet, DOTA-v2, FAIR1M, Geochat-Instruction(only related to DOTA, DIOR, FAIR1M) \\
RS-LLaVA~\cite{rs-llava} & 7058 & Image Caption, VQA & UCM-captions, UAV, RSVQA-LR, RSIVQA-DOTA \\
Popeye~\cite{popeye} & 81k & Ship Detection & DOSR, DOTA ship subset, SSDD, HRSID \\
\bottomrule

\end{tabularx}
\vspace{-5pt}
\end{table}
